Impact of Data Poisoning Attacks on Feasibility and Optimality of Neural Power System Optimizers

The increased integration of clean yet stochastic energy resources and the growing number of extreme weather events are narrowing the decision-making window of power grid operators. This time constraint is fueling a plethora of research on Machine Learning-, or ML-, based optimization proxies. While finding a fast solution is appealing, the inherent vulnerabilities of the learning-based methods are hindering their adoption. One of these vulnerabilities is data poisoning attacks, which adds perturbations to ML training data, leading to incorrect decisions. The impact of poisoning attacks on learning-based power system optimizers have not been thoroughly studied, which creates a critical vulnerability. In this paper, we examine the impact of data poisoning attacks on ML-based optimization proxies that are used to solve the DC Optimal Power Flow problem. Specifically, we compare the resilience of three different methods-a penalty-based method, a post-repair approach, and a direct mapping approach-against the adverse effects of poisoning attacks. We will use the optimality and feasibility of these proxies as performance metrics. The insights of this work will establish a foundation for enhancing the resilience of neural power system optimizers.

==> Reviewer_comments.tex <==
\begin{document}
----------------------- REVIEW 1 ---------------------
SUBMISSION: 69
TITLE: Impact of Data Poisoning Attacks on Feasibility and Optimality of Neural Power System Optimizers
AUTHORS: Nora Agah, Meiyi Li and Javad Mohammadi

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
The paper is in the scope of a practical field, however, the following considerations made:

[Presentation and Writing]

1- The introduction should be systematic which means context to the field, importance of the field, a mini literature review of the field, then gap, and finally, your contributions, and paper structure.
2- Figures should be in Times New Roman font, and be inserted in vector (SVG) to the paper, avoiding lack of quality.
3- The equations 1a to 1f should be 1.1 to 1.6
4- There are undefined abbreviations. For example, in the abstract, you have used Machine Learning, and ML. So you have not defined ML as Machine Learning (ML). Recheck for all undefined ones.
5- The functionality of the clip function is not ordered. It should be equation (4).
6- Instead of using <we> pronoun and active voice sentences, use passive voice sentences. It is the professional way.

[Technical]

1- Considering the computation complexity (CC), just time is considered in Table 1. The authors should consider the other CC important factors. Then, re-conduct the comparison.
2- What the authors did, in this paper, is mainly about data-driven simulations. So, it cannot be considered as experimental setup. Consequently, <Simulation> is a better candidate instead of <Experimental>. Regarding this, update the words.
3- From 21 references, just 3 of them are 2024. the authors should use more recent works instead.
4- The upper and lower boundaries numerical values of the terms are not presented in the paper. Should be clarified.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 69
TITLE: Impact of Data Poisoning Attacks on Feasibility and Optimality of Neural Power System Optimizers
AUTHORS: Nora Agah, Meiyi Li and Javad Mohammadi

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The paper focuses on a critical yet under-researched vulnerability in ML-based power system optimizers-data poisoning attacks. It is a highly relevant study considering the increasing reliance on ML for real-time decision-making in power grids.

The comparison of the three approaches—Penalty-based, DC3, and LOOP-LC—is clear and systematic. The focus on both feasibility and optimality metrics strengthens the rigor of the study.

The experimental results are presented in detail with clear visualizations, such as that in Fig. 4, and a concise summary in Table I. The metrics such as optimality gap, feasibility gap, and CPU time effectively provide a holistic view of the performance.

These include extension proposals for the development of poisoning attacks for AC-OPF and the incorporation of adversarial defenses.

Include a clearer motivation for choosing data poisoning over evasion attacks, emphasizing why this threat is particularly critical for grid optimization compared to operational phase attacks.

Add a few recent works (2023–2024) on adversarial robustness in ML-based power systems to highlight state-of-the-art methods that deal with vulnerabilities.

Discuss mitigation techniques like adversarial training or robust optimization briefly to contextualize the importance of this study further.

Improve the labels and legends of the graphs in Fig. 4 for readability purposes. For example, placing units where appropriate and bolding titles to the axes will enhance this. Ensure that legends appear the same way in all plots of Fig. 4 for consistency.

State your reason for choosing a perturbation bound of 0.75 instead of any other. Present a short justification.

Make practical implications more explicit, as in how grid operators might apply this work toward making their system more resilient against adversarial attacks.

Use uniform citation style for all references. For instance, the DOIs must be formatted properly.


\end{document}

==> outline.tex <==
Motiviation
1. Introduce grid. Grid changes-more variables (renewables), more extreme weather events, more decisions to be made - grid is facing these challenges and it is difficult to balance supply and demand and power system operations, for example in OPF?
2.Traditional iterative solvers are slow. Need to resolve every 15 mins. We have a lot of historical data that can be used to train. AI solvers is needed in the grid. 
3. Operators are hesitant also to use AI methods because of uncertainty of the risk. The risks that come with AI solvers, important to explore things like poisoning to understand and improve robustness

Literature Review
1. Existing AI optimization proxies
2. Poisoning literature review in application to power systems 
3. Emphasize gap in poisoning of power systems methods

Contribution
1. Determining the impact of poisoning attacks on new power grid AI solvers
2. Giving guide to increase robustness of future solvers and ways to modify current solvers to be more robust


Problem Formulation
1. DCOPF
This is about the formultion. Define the mathematical formulation. 
2. Explain how AI Solvers for DCOPF work.
3. Poisoning explanation and formulation

AI Method Overview
1. Penalty
2. LOOP-LC
3. DC3

Results
Explain experiment setup-like dataset 
Give the metrics-how we calc feasibility and optimality gap

Provide tables and figures-give one showing the trenf of eps and error?

Conclusion
1.Our observations from the results. There is an impact! This can cause many problems 
2. Future directions - ACOPF, training or modifying for robustness, more methods



